Learning Probability Distributions in Macroeconomics and Finance

We propose a deep learning approach to probabilistic forecasting of macroeconomic and financial time series. Being able to learn complex patterns from a data rich environment, our approach is useful for a decision making that depends on uncertainty of large number of economic outcomes. Specifically, it is informative to agents facing asymmetric dependence of their loss on outcomes from possibly non-Gaussian and non-linear variables. We show the usefulness of the proposed approach on the two distinct datasets where a machine learns the pattern from data. First, we construct macroeconomic fan charts that reflect information from high-dimensional data set. Second, we illustrate gains in prediction of stock return distributions which are heavy tailed, asymmetric and suffer from low signal-to-noise ratio.

==> figsMacro/15_macro/diebold_mariano_table_2022-03-30.tex <==
\begin{table}
  \caption{Table: 2, Diebold Mariano test, ML vs BVAR}
  \begin{tabular}{rrrrrr}
    \hline\hline
     & \textbf{0.1 DM ML not worse} & \textbf{0.25 DM ML not worse} & \textbf{0.5 DM ML not worse} & \textbf{0.75 DM ML not worse} & \textbf{0.9 DM ML not worse} \\\hline
    GDP h=1 & 0.5907 & -0.1721 & -0.4901 & 0.1888 & -1.004 \\
    GDP h=2 & \color{blue}{\textbf{-2.847 *** }} & -0.5012 & 0.3416 & 0.1301 & -0.6873 \\
    GDP h=3 & 0.1281 & -0.5745 & -0.6872 & -1.195 & -0.7747 \\
    GDP h=4 & 0.3385 & -0.22 & -0.8577 & -1.191 & -1.207 \\
    GDP h=5 & -1.547 & -0.9693 & -1.096 & -1.207 & -0.87 \\
    GDP h=6 & 0.7251 & 0.9663 & 0.6626 & \color{blue}{\textbf{1.827 * }} & -0.5057 \\\hline
    CPI h=1 & -0.000865 & -0.02898 & -0.5032 & -0.7995 & -1.655 \\
    CPI h=2 & -0.008789 & 0.184 & 0.5168 & -0.269 & \color{blue}{\textbf{-2.372 **}} \\
    CPI h=3 & 0.5859 & 0.09548 & 0.5499 & -0.6472 & \color{blue}{\textbf{-2.902 *** }} \\
    CPI h=4 & -0.2778 & 0.003453 & 0.7932 & -0.1922 & -1.514 \\
    CPI h=5 & \color{blue}{\textbf{-3.423 *** }} & 0.8616 & 1.136 & -0.608 & \color{blue}{\textbf{-3.229 *** }} \\
    CPI h=6 & 1.415 & 1.232 & 0.5057 & -1.1 & \color{blue}{\textbf{-3.323 *** }} \\\hline
    UNE h=1 & -1.388 & -0.9667 & -1.273 & -0.9143 & -1.36 \\
    UNE h=2 & -0.0847 & -0.4339 & -1.068 & -0.281 & -0.6747 \\
    UNE h=3 & 1.3 & -0.7421 & \color{blue}{\textbf{-1.911 * }} & -0.7944 & -0.6751 \\
    UNE h=4 & 1.472 & 0.3844 & -0.5832 & -0.1421 & -0.5993 \\
    UNE h=5 & \color{blue}{\textbf{-4.064 *** }} & -0.7075 & -1.5 & -0.8157 & -0.6481 \\
    UNE h=6 & \color{blue}{\textbf{2.113 **}} & 1.653 & -1.672 & -0.9107 & -1.423 \\\hline\hline
  \end{tabular}
\end{table}


==> figsMacro/15_macro/loss_latex_table_2022-03-30.tex <==
\begin{table}
  \caption{Table: 1, ML has lower quantile loss than BVAR}
  \begin{tabular}{rrrrrrrrrrr}
    \hline\hline
     & \textbf{0.1 ML} & \textbf{0.1 BVAR} & \textbf{0.25 ML} & \textbf{0.25 BVAR} & \textbf{0.5 ML} & \textbf{0.5 BVAR} & \textbf{0.75 ML} & \textbf{0.75 BVAR} & \textbf{0.9 ML} & \textbf{0.9 BVAR} \\\hline
    GDP h=1 & 2.469 & 2.146 & \color{blue}{\textbf{3.535*}} & 3.645 & \color{blue}{\textbf{4.004*}} & 4.28 & 3.125 & 3.06 & \color{blue}{\textbf{1.839*}} & 2.381 \\
    GDP h=2 & \color{blue}{\textbf{1.699*}} & 2.305 & \color{blue}{\textbf{3.305*}} & 3.478 & 3.906 & 3.671 & 3.132 & 3.026 & \color{blue}{\textbf{2.025*}} & 2.665 \\
    GDP h=3 & 2.262 & 2.193 & \color{blue}{\textbf{3.289*}} & 3.51 & \color{blue}{\textbf{3.714*}} & 4.307 & \color{blue}{\textbf{2.551*}} & 3.203 & \color{blue}{\textbf{1.776*}} & 2.363 \\
    GDP h=4 & 2.321 & 2.13 & \color{blue}{\textbf{3.502*}} & 3.626 & \color{blue}{\textbf{3.888*}} & 4.513 & \color{blue}{\textbf{2.81*}} & 3.349 & \color{blue}{\textbf{1.598*}} & 2.679 \\
    GDP h=5 & \color{blue}{\textbf{1.717*}} & 2.199 & \color{blue}{\textbf{2.877*}} & 3.193 & \color{blue}{\textbf{3.64*}} & 4.222 & \color{blue}{\textbf{2.889*}} & 3.188 & \color{blue}{\textbf{1.765*}} & 2.546 \\
    GDP h=6 & 2.768 & 2.159 & 3.778 & 3.036 & 4.343 & 4.066 & 3.591 & 3.061 & \color{blue}{\textbf{2.089*}} & 2.374 \\\hline
    CPI h=1 & \color{blue}{\textbf{4.05*}} & 4.051 & \color{blue}{\textbf{6.836*}} & 6.884 & \color{blue}{\textbf{8.862*}} & 9.509 & \color{blue}{\textbf{7.388*}} & 8.552 & \color{blue}{\textbf{4.746*}} & 7.925 \\
    CPI h=2 & \color{blue}{\textbf{3.098*}} & 3.102 & 5.986 & 5.864 & 8.885 & 8.411 & \color{blue}{\textbf{8.241*}} & 8.611 & \color{blue}{\textbf{4.918*}} & 8.65 \\
    CPI h=3 & 3.408 & 3.171 & 5.359 & 5.295 & 8.227 & 7.937 & \color{blue}{\textbf{7.691*}} & 8.252 & \color{blue}{\textbf{5.09*}} & 8.453 \\
    CPI h=4 & \color{blue}{\textbf{2.839*}} & 2.955 & 5.598 & 5.596 & 8.909 & 8.399 & \color{blue}{\textbf{7.882*}} & 8.169 & \color{blue}{\textbf{4.587*}} & 8.21 \\
    CPI h=5 & \color{blue}{\textbf{2.514*}} & 3.037 & 5.947 & 5.261 & 8.966 & 7.944 & \color{blue}{\textbf{7.589*}} & 8.102 & \color{blue}{\textbf{4.803*}} & 8.101 \\
    CPI h=6 & 4.183 & 3.055 & 6.892 & 5.215 & 8.206 & 7.85 & \color{blue}{\textbf{7.417*}} & 8.006 & \color{blue}{\textbf{4.579*}} & 8.178 \\\hline
    UNE h=1 & \color{blue}{\textbf{1.528*}} & 2.182 & \color{blue}{\textbf{2.98*}} & 3.718 & \color{blue}{\textbf{3.687*}} & 4.799 & \color{blue}{\textbf{2.934*}} & 3.495 & \color{blue}{\textbf{1.538*}} & 2.634 \\
    UNE h=2 & \color{blue}{\textbf{2.273*}} & 2.359 & \color{blue}{\textbf{3.469*}} & 4.022 & \color{blue}{\textbf{3.669*}} & 4.814 & \color{blue}{\textbf{2.982*}} & 3.155 & \color{blue}{\textbf{1.646*}} & 2.168 \\
    UNE h=3 & 2.486 & 1.956 & \color{blue}{\textbf{3.187*}} & 3.753 & \color{blue}{\textbf{3.559*}} & 5.128 & \color{blue}{\textbf{2.954*}} & 3.563 & \color{blue}{\textbf{1.929*}} & 2.614 \\
    UNE h=4 & 3.095 & 1.841 & 4.275 & 3.666 & \color{blue}{\textbf{4.77*}} & 5.6 & \color{blue}{\textbf{3.632*}} & 3.769 & \color{blue}{\textbf{2.235*}} & 2.735 \\
    UNE h=5 & \color{blue}{\textbf{1.502*}} & 1.91 & \color{blue}{\textbf{3.168*}} & 3.851 & \color{blue}{\textbf{4.003*}} & 5.777 & \color{blue}{\textbf{3.449*}} & 3.851 & \color{blue}{\textbf{2.242*}} & 2.621 \\
    UNE h=6 & 3.292 & 1.916 & 4.404 & 3.751 & \color{blue}{\textbf{4.589*}} & 5.776 & \color{blue}{\textbf{3.445*}} & 3.728 & \color{blue}{\textbf{2.039*}} & 2.518 \\\hline\hline
  \end{tabular}
\end{table}


==> figsMacro/19_macro/diebold_mariano_table_2022-03-30.tex <==
\begin{table}
  \caption{Table: 2, Diebold Mariano test, ML vs BVAR}
  \begin{tabular}{rrrrrr}
    \hline\hline
     & \textbf{0.1 DM ML not worse} & \textbf{0.25 DM ML not worse} & \textbf{0.5 DM ML not worse} & \textbf{0.75 DM ML not worse} & \textbf{0.9 DM ML not worse} \\\hline
    GDP h=1 & -0.4234 & \color{blue}{\textbf{-2.0609 * }} & -0.8421 & 0.1479 & -1.0619 \\
    GDP h=2 & -0.1094 & -0.4939 & 0.5027 & -0.2906 & -0.9199 \\
    GDP h=3 & 0.1516 & -0.0821 & -0.0757 & 0.5351 & -0.0948 \\
    GDP h=4 & -0.8808 & -1.6944 & -0.6268 & -0.9966 & -1.1122 \\
    GDP h=5 & -1.4336 & -0.4723 & -0.4374 & \color{blue}{\textbf{-2.5705 **}} & -1.3932 \\
    GDP h=6 & 0.0508 & 0.8273 & -0.3862 & -0.6077 & -0.5314 \\\hline
    CPI h=1 & -0.0369 & -0.5153 & -1.6002 & -0.8522 & \color{blue}{\textbf{-1.718 * }} \\
    CPI h=2 & 0.7832 & 0.5475 & 0.1647 & -1.1302 & \color{blue}{\textbf{-3.1631 *** }} \\
    CPI h=3 & \color{blue}{\textbf{-4.7111 *** }} & 0.0436 & 1.0352 & 0.0345 & \color{blue}{\textbf{-2.1701 **}} \\
    CPI h=4 & -0.3859 & 0.3249 & 0.151 & -0.9863 & \color{blue}{\textbf{-1.7402 * }} \\
    CPI h=5 & 0.5635 & \color{blue}{\textbf{3.9307 *** }} & 0.101 & \color{blue}{\textbf{-5.553 *** }} & \color{blue}{\textbf{-14.7935 *** }} \\
    CPI h=6 & 0.8104 & 1.5175 & 0.2902 & -1.0714 & \color{blue}{\textbf{-2.1468 **}} \\\hline
    UNE h=1 & -0.3937 & -0.8682 & \color{blue}{\textbf{-1.7259 * }} & -1.0862 & -1.2746 \\
    UNE h=2 & -0.9097 & -1.3733 & -1.5014 & -0.2501 & -0.4865 \\
    UNE h=3 & -0.1361 & -0.4044 & -1.4017 & 0.0155 & -0.1076 \\
    UNE h=4 & 0.8105 & 0.0321 & -1.3888 & -0.4531 & -0.5153 \\
    UNE h=5 & 1.479 & -0.0008 & -1.1089 & -0.7159 & -1.1653 \\
    UNE h=6 & 1.1521 & -0.6429 & \color{blue}{\textbf{-2.0862 **}} & -1.7029 & -1.6384 \\\hline\hline
  \end{tabular}
\end{table}


==> figsMacro/19_macro/loss_latex_table_2022-03-30.tex <==
\begin{table}
  \caption{Table: 1, ML has lower quantile loss than BVAR, N of better 65/90}
  \begin{tabular}{rrrrrrrrrrr}
    \hline\hline
     & \textbf{0.1 ML} & \textbf{0.1 BVAR} & \textbf{0.25 ML} & \textbf{0.25 BVAR} & \textbf{0.5 ML} & \textbf{0.5 BVAR} & \textbf{0.75 ML} & \textbf{0.75 BVAR} & \textbf{0.9 ML} & \textbf{0.9 BVAR} \\\hline
    GDP h=1 & \color{blue}{\textbf{1.985*}} & 2.146 & \color{blue}{\textbf{2.829*}} & 3.645 & \color{blue}{\textbf{3.751*}} & 4.28 & 3.118 & 3.06 & \color{blue}{\textbf{1.917*}} & 2.381 \\
    GDP h=2 & \color{blue}{\textbf{2.253*}} & 2.305 & \color{blue}{\textbf{3.338*}} & 3.478 & 3.957 & 3.671 & \color{blue}{\textbf{2.8*}} & 3.026 & \color{blue}{\textbf{1.826*}} & 2.665 \\
    GDP h=3 & 2.317 & 2.193 & \color{blue}{\textbf{3.444*}} & 3.51 & \color{blue}{\textbf{4.249*}} & 4.307 & 3.524 & 3.203 & \color{blue}{\textbf{2.287*}} & 2.363 \\
    GDP h=4 & \color{blue}{\textbf{1.977*}} & 2.13 & \color{blue}{\textbf{3.437*}} & 3.626 & \color{blue}{\textbf{4.013*}} & 4.513 & \color{blue}{\textbf{2.931*}} & 3.349 & \color{blue}{\textbf{1.71*}} & 2.679 \\
    GDP h=5 & \color{blue}{\textbf{1.843*}} & 2.199 & \color{blue}{\textbf{3.141*}} & 3.193 & \color{blue}{\textbf{3.85*}} & 4.222 & \color{blue}{\textbf{2.564*}} & 3.188 & \color{blue}{\textbf{1.549*}} & 2.546 \\
    GDP h=6 & 2.176 & 2.159 & 3.298 & 3.036 & \color{blue}{\textbf{3.776*}} & 4.066 & \color{blue}{\textbf{2.682*}} & 3.061 & \color{blue}{\textbf{1.909*}} & 2.374 \\\hline
    CPI h=1 & \color{blue}{\textbf{4.017*}} & 4.051 & \color{blue}{\textbf{6.294*}} & 6.884 & \color{blue}{\textbf{7.711*}} & 9.509 & \color{blue}{\textbf{7.373*}} & 8.552 & \color{blue}{\textbf{4.472*}} & 7.925 \\
    CPI h=2 & 3.408 & 3.102 & 6.339 & 5.864 & 8.554 & 8.411 & \color{blue}{\textbf{7.325*}} & 8.611 & \color{blue}{\textbf{3.959*}} & 8.65 \\
    CPI h=3 & \color{blue}{\textbf{2.509*}} & 3.171 & 5.319 & 5.295 & 8.394 & 7.937 & 8.291 & 8.252 & \color{blue}{\textbf{5.574*}} & 8.453 \\
    CPI h=4 & \color{blue}{\textbf{2.899*}} & 2.955 & 5.889 & 5.596 & 8.481 & 8.399 & \color{blue}{\textbf{7.485*}} & 8.169 & \color{blue}{\textbf{5.023*}} & 8.21 \\
    CPI h=5 & 3.454 & 3.037 & 5.973 & 5.261 & 8.004 & 7.944 & \color{blue}{\textbf{7.138*}} & 8.102 & \color{blue}{\textbf{4.941*}} & 8.101 \\
    CPI h=6 & 4.004 & 3.055 & 6.747 & 5.215 & 8.198 & 7.85 & \color{blue}{\textbf{6.941*}} & 8.006 & \color{blue}{\textbf{4.645*}} & 8.178 \\\hline
    UNE h=1 & \color{blue}{\textbf{1.95*}} & 2.182 & \color{blue}{\textbf{3.06*}} & 3.718 & \color{blue}{\textbf{3.586*}} & 4.799 & \color{blue}{\textbf{2.928*}} & 3.495 & \color{blue}{\textbf{1.639*}} & 2.634 \\
    UNE h=2 & \color{blue}{\textbf{1.86*}} & 2.359 & \color{blue}{\textbf{3.126*}} & 4.022 & \color{blue}{\textbf{3.703*}} & 4.814 & \color{blue}{\textbf{2.995*}} & 3.155 & \color{blue}{\textbf{1.794*}} & 2.168 \\
    UNE h=3 & \color{blue}{\textbf{1.902*}} & 1.956 & \color{blue}{\textbf{3.407*}} & 3.753 & \color{blue}{\textbf{4.004*}} & 5.128 & 3.579 & 3.563 & \color{blue}{\textbf{2.486*}} & 2.614 \\
    UNE h=4 & 2.605 & 1.841 & 3.712 & 3.666 & \color{blue}{\textbf{3.884*}} & 5.6 & \color{blue}{\textbf{3.252*}} & 3.769 & \color{blue}{\textbf{2.193*}} & 2.735 \\
    UNE h=5 & 2.187 & 1.91 & \color{blue}{\textbf{3.851*}} & 3.851 & \color{blue}{\textbf{4.383*}} & 5.777 & \color{blue}{\textbf{3.263*}} & 3.851 & \color{blue}{\textbf{1.816*}} & 2.621 \\
    UNE h=6 & 2.113 & 1.916 & \color{blue}{\textbf{3.253*}} & 3.751 & \color{blue}{\textbf{3.731*}} & 5.776 & \color{blue}{\textbf{2.929*}} & 3.728 & \color{blue}{\textbf{1.756*}} & 2.518 \\\hline\hline
  \end{tabular}
\end{table}

